Hidden in Plain Sight: Evaluation of the Deception Detection Capabilities of LLMs in Multimodal Settings

Detecting deception in an increasingly digital world is both a critical and challenging task. In this study, we present a comprehensive evaluation of the automated deception detection capabilities of Large Language Models (LLMs) and Large Multimodal Models (LMMs) across diverse domains. We assess the performance of both open-source and commercial LLMs on three distinct datasets: real life trial interviews (RLTD), instructed deception in interpersonal scenarios (MU3D), and deceptive reviews (OpSpam). We systematically analyze the effectiveness of different experimental setups for deception detection, including zero-shot and few-shot approaches with random or similarity-based in-context example selection. Our results show that fine-tuned LLMs achieve state-of-the-art performance on textual deception detection tasks, while LMMs struggle to fully leverage cross-modal cues. Additionally, we analyze the impact of auxiliary features, such as non-verbal gestures and video summaries, and examine the effectiveness of different prompting strategies, including direct label generation and chain-of-thought reasoning. Our findings provide key insights into how LLMs process and interpret deceptive cues across modalities, highlighting their potential and limitations in real-world deception detection applications.

==> latex/tables/table_1.tex <==
\begin{table*}[ht]
\centering

\begin{tabular}{l c cc cc cc}
\toprule
\multirow{2}{*}{\textbf{Baseline}} & \multirow{2}{*}{\textbf{Modality}} 
  & \multicolumn{2}{c}{\textbf{RLTD}} 
  & \multicolumn{2}{c}{\textbf{MU3D}} 
  & \multicolumn{2}{c}{\textbf{OpSpam}} \\
& & \textbf{acc} & \textbf{f1} & \textbf{acc} & \textbf{f1} & \textbf{acc} & \textbf{f1} \\
\midrule
  RoBERTa-ft 
  & t        & 76.31 & 76.22 & 67.92 & 67.81 & 88.10 & 88.09 \\
\midrule
\multirow{4}{*}{BiLSTM+Attention} 
  & t        & 69.42 & 69.37 & 65.94 & 65.76 & 90.45 & 90.45 \\
  & a        & 68.04 & 68.02 & 62.19 & 61.82 & -     & -     \\
  & v        & 75.48 & 75.38 & 55.21 & 55.11 & -     & -     \\
  & t, a, v    & 77.14 & 77.04 & 62.29 & 62.19 & -     & -     \\
\midrule
\multirow{4}{*}{CNN}
  & t        & 64.46 & 64.39 & 64.06 & 63.91 & 86.37 & 86.36 \\
  & a        & 60.88 & 60.13 & 60.42 & 60.26 & -     & -     \\
  & v        & 82.09 & 82.09 & 54.06 & 53.95 & -     & -     \\
  & t, a, v    & 83.47 & 83.44 & 60.41 & 60.38 & -     & -     \\
\midrule
PECL 
  & a, v      & 80.17 & 80.13 & 56.56 & 56.56 & -     & -     \\
\bottomrule
\end{tabular}
\captionsetup{font=scriptsize}
\caption{Results on RLTD, MU3D, and OpSpam datasets.}
\label{tab:myresults}
\end{table*}

